Let's Ask Again: Refine Network for Automatic Question Generation

In this work, we focus on the task of Automatic Question Generation (AQG) where given a passage and an answer the task is to generate the corresponding question. It is desired that the generated question should be (i) grammatically correct (ii) answerable from the passage and (iii) specific to the given answer. An analysis of existing AQG models shows that they produce questions which do not adhere to one or more of {the above-mentioned qualities}. In particular, the generated questions look like an incomplete draft of the desired question with a clear scope for refinement. {To alleviate this shortcoming}, we propose a method which tries to mimic the human process of generating questions by first creating an initial draft and then refining it. More specifically, we propose Refine Network (RefNet) which contains two decoders. The second decoder uses a dual attention network which pays attention to both (i) the original passage and (ii) the question (initial draft) generated by the first decoder. In effect, it refines the question generated by the first decoder, thereby making it more correct and complete. We evaluate RefNet on three datasets, \textit{viz.}, SQuAD, HOTPOT-QA, and DROP, and show that it outperforms existing state-of-the-art methods by 7-16\% on all of these datasets. Lastly, we show that we can improve the quality of the second decoder on specific metrics, such as, fluency and answerability by explicitly rewarding revisions that improve on the corresponding metric during training. The code has been made publicly available \footnote{https://github.com/PrekshaNema25/RefNet-QG}

==> notused/all_datasets1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\resizebox{\textwidth}{!}{
\begin{tabular}{l|lllllll|l}
\hline\hline
\multirow{2}{*}{\textbf{Dataset}}                                                          & \multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{6}{c|}{\textbf{n-gram}}                                                                                                                                                                         &  \\ \cline{3-8} 
                                                                                           & \multicolumn{1}{l|}{}                                & \multicolumn{1}{l|}{BLEU-1}         & \multicolumn{1}{l|}{BLEU-2}         & \multicolumn{1}{l|}{BLEU-3}         & \multicolumn{1}{l|}{BLEU-4}         & \multicolumn{1}{l|}{ROUGE-L}        & METEOR         &  QBLEU4               \\ \hline\hine
\multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}SQuAD\\ (Sent. Level)\end{tabular}}} 
  &                           \multicolumn{1}{l|}{\cite{answerfocuesdqg}}                          & \multicolumn{1}{l}{43.02}          & \multicolumn{1}{l}{28.14}          & \multicolumn{1}{l}{20.51}          & \multicolumn{1}{l}{15.64}          & \multicolumn{1}{l}{-}          & -         & -                  \\ 
   &                           \multicolumn{1}{l|}{\cite{para}}                         & \multicolumn{1}{l}{44.51}          & \multicolumn{1}{l}{29.07}          & \multicolumn{1}{l}{21.06}          & \multicolumn{1}{l}{15.82}          & \multicolumn{1}{l}{44.24}          & 19.67          & -                 \\ 
   &                           \multicolumn{1}{l|}{\cite{Kim2019ImprovingNQ}}                          & \multicolumn{1}{l}{-}          & \multicolumn{1}{l}{-}          & \multicolumn{1}{l}{-}          & \multicolumn{1}{l}{16.17}          & \multicolumn{1}{l}{-}          & -         & -                  \\ \cline{2-9}




                                                                & \multicolumn{1}{l|}{EAD}                             & \multicolumn{1}{l}{44.74}          & \multicolumn{1}{l}{29.79}          & \multicolumn{1}{l}{22.00}          & \multicolumn{1}{l}{16.84}          & \multicolumn{1}{l}{44.78}          & 20.60          & 24.7                  \\
                                                                                         
                                                                 &                           \multicolumn{1}{l|}{RefNet}                          & \multicolumn{1}{l}{\textbf{47.27}}          & \multicolumn{1}{l}{\textbf{31.88}}          & \multicolumn{1}{l}{\textbf{23.65}}          & \multicolumn{1}{l}{\textbf{18.16}}          & \multicolumn{1}{l}{\textbf{47.14}}          & \textbf{23.40}          & \textbf{27.4}                  \\ 
                                 %       & \multicolumn{1}{l|}{RefNet + BLEU}                   & \multicolumn{1}{l}{\textbf{48.17}} & \multicolumn{1}{l}{\textbf{32.49}} & \multicolumn{1}{l}{\textbf{24.12}} & \multicolumn{1}{l}{\textbf{18.52}} & \multicolumn{1}{l}{\textbf{47.56}} & 23.49          & 27.60                  \\
                                                                   %                        & \multicolumn{1}{l|}{RefNet + QBleu}                  & \multicolumn{1}{l}{47.49}          & \multicolumn{1}{l}{32.03}          & \multicolumn{1}{l}{23.74}          & \multicolumn{1}{l}{18.17}          & \multicolumn{1}{l}{47.88}          & \textbf{23.87} & \textbf{28.60}         \\                            
                                                                                  \hline\hline
                                                                                        
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}SQuAD\\ (Psg. Level)\end{tabular}}}  
                                                     &                           \multicolumn{1}{l|}{\cite{para}}                          & \multicolumn{1}{l}{45.07}          & \multicolumn{1}{l}{29.58}          & \multicolumn{1}{l}{21.60}          & \multicolumn{1}{l}{16.38}          & \multicolumn{1}{l}{44.48}          & 20.25          & -                  \\ \cline{2-9}





& \multicolumn{1}{l|}{EAD}                             & \multicolumn{1}{l}{44.61}          & \multicolumn{1}{l}{29.37}          & \multicolumn{1}{l}{21.50}          & \multicolumn{1}{l}{16.36}          & \multicolumn{1}{l}{43.95}          & 20.11         & 24.2                  \\
     & \multicolumn{1}{l|}{RefNet}                          & \multicolumn{1}{l}{\textbf{46.41}}          & \multicolumn{1}{l}{\textbf{30.66}}          & \multicolumn{1}{l}{\textbf{22.42}}          & \multicolumn{1}{l}{\textbf{16.99}}          & \multicolumn{1}{l}{\textbf{45.03}}          & \textbf{21.10}          & \textbf{26.6}                  \\

                                                                    %                     & \multicolumn{1}{l|}{RefNet + BLEU}                   & \multicolumn{1}{l}{46.66}          & \multicolumn{1}{l}{30.85}          & \multicolumn{1}{l}{22.56}          & \multicolumn{1}{l}{17.11}          & \multicolumn{1}{l}{45.35}          & 21.24          & 27.0                   \\
                                                                     %                      & \multicolumn{1}{l|}{RefNet + QBLEu}                  & \multicolumn{1}{l}{\textbf{46.83}} & \multicolumn{1}{l}{\textbf{31.08}} & \multicolumn{1}{l}{\textbf{22.76}} & \multicolumn{1}{l}{\textbf{17.24}} & \multicolumn{1}{l}{45.66}          & \textbf{21.32} & \textbf{27.20}         \\
                                                                                           %& %\multicolumn{1}{l|}{EAD + BLEU}                      & \multicolumn{1}{l|}{}               & \multicolumn{1}{l|}{}               & \multicolumn{1}{l|}{}               & \multicolumn{1}{l|}{}               & \multicolumn{1}{l|}{}               &                &                        \\
                                                                                           %& %\multicolumn{1}{l|}{EAD + QBLEU}                     & \multicolumn{1}{l|}{44.48}               & \multicolumn{1}{l|}{29.70}               & \multicolumn{1}{l|}{21.94}               & \multicolumn{1}{l|}{16.83}               & \multicolumn{1}{l|}{45.03}               &  20.63              &    25.4                   \\
                                                                                        %   & %\multicolumn{1}{l|}{EAD + Original}                  & \multicolumn{1}{l|}{43.17}          & \multicolumn{1}{l|}{28.24}          & \multicolumn{1}{l|}{20.52}          & \multicolumn{1}{l|}{15.52}          & \multicolumn{1}{l|}{43.96}          & 19.74         & 24.20                  \\ \cline{2-9} 
                                                            
                                                            \hline\hline
                                                    
\multirow{3}{*}{\textbf{HOTPOT}} &                           \multicolumn{1}{l|}{\cite{para}*}                          & \multicolumn{1}{l}{45.29}          & \multicolumn{1}{l}{32.06}          & \multicolumn{1}{l}{24.43}          & \multicolumn{1}{l}{19.29}          & \multicolumn{1}{l}{40.40}          & 19.29         & 25.7              \\ \cline{2-9}

& \multicolumn{1}{l|}{EAD}                                                            & 46.00         & 32.47          & 24.82          & 19.68          & 41.52          & 23.27          &     26.2               \\
                                       & \multicolumn{1}{l|}{RefNet}                                                          & \textbf{45.45}          & \textbf{33.13}          & \textbf{26.05}          & \textbf{21.17}          & \textbf{43.12}          & \textbf{25.81}          & \textbf{28.7}  \\
                                    %& \multicolumn{1}{l|}{RefNet + BLEU}                                                   & \textbf{}      & \textbf{}      & \textbf{}      & \textbf{}      & \textbf{}      &                &                        \\
                                     %  & \multicolumn{1}{l|}{RefNet + QBleu}                                                  & \textbf{47.96} & \textbf{34.62} & \textbf{26.82} & \textbf{21.48} & \textbf{43.35} & \textbf{25.03} & \textbf{31.4} 
                                       \hline\hline
\multirow{3}{*}{\textbf{DROP Dataset}} &                           \multicolumn{1}{l|}{\cite{para}*}                          & \multicolumn{1}{l}{39.56}          & \multicolumn{1}{l}{29.19}          & \multicolumn{1}{l}{22.53}          & \multicolumn{1}{l}{18.07}          & \multicolumn{1}{l}{45.01}          & 19.68          & 31.4                 \\ \cline{2-9}


&\multicolumn{1}{l|}{EAD}                                                            & 39.21          & 29.10          & 22.65          & 18.42          & 45.07          & 19.56          & 31.8                 \\
                                       & \multicolumn{1}{l|}{RefNet}                                                    & \textbf{42.81}          & \textbf{32.63}          & \textbf{25.78}          & \textbf{21.23}          & \textbf{47.49 }         & \textbf{22.25}          &  \textbf{33.6 }                 \\
                                      %     & \multicolumn{1}{l|}{Reinforce Revision(BLEU)}                                               & \textbf{42.82} & \textbf{32.83} & \textbf{26.12} & \textbf{21.60} & \textbf{48.16} & \textbf{22.43} & \textbf{34.3}          \\
                                      % & \multicolumn{1}{l|}{Reinforce Revision(QBLEU)}                                                 & 42.66          & 32.73          & 26.06          & 21.59          & 47.83          & 22.29          & 34.1  \\                                   \hline\hline
                                       
%\multirow{2}{*}{\textbf{MS-Marco}}     & \multicolumn{1}{l|}{EAD}                                                           & 46.66          & 30.85          & 22.56          & 17.11          & 45.35          & 21.24          & 27.0                   \\
 %                                      &\multicolumn{1}{l|}{RefNet}                                                       & 46.00 & 33.02 & 24.05 & 18.00 & 48.02          & 23.80 & 27.8          \\ \hline
\hline\hline
\end{tabular}}
\caption{Comparsion of RefNet model with existing approaches and EAD model. * denotes our implementation of the corresponding work.}
\label{tab:results1}
\end{table*}

==> notused/result_table_across_datasets_ngram.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\resizebox{\textwidth}{!}{  
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{Dataset}}    & \multirow{2}{*}{\textbf{Model}} & \multicolumn{6}{c|}{\textbf{$n$-gram metrics}}                                                             & \textbf{\begin{tabular}[c]{@{}l@{}}Answer-\\ ability\end{tabular}} \\ \cline{3-9} 
                                     &                                 & \textbf{BLEU-1} & \textbf{BLEU-2} & \textbf{BLEU-3} & \textbf{BLEU-4} & \textbf{ROUGE-L} & \textbf{METEOR} & \multicolumn{1}{c|}{\textbf{QBLEU-4}}                              \\ \hline
\multirow{5}{*}{\textbf{SQuAD v1.1}} & \cite{learningtoask}                              & 43.09           & 25.96           & 17.50           & 12.28           & 39.75            & 16.62           & -                                                                  \\ 
                                     & \cite{Song2017AUQ}                             & -               & -               & -               & 13.98           & 42.72            & 18.77           & -                                                                  \\ 
                                     & \cite{para}^*            & 43.47           & 28.23           & 20.40           & 15.32           & 43.91            & 19.29           & -                                                                  \\ 
                                     & EAD Model                & 43.77           & 28.70           & 20.92           & 15.82           & 43.70            & 20.97           & 24.9                                                               \\ 
                                     & \textbf{RevNet Model}     & 46.30  & 30.80  & 22.59  & 17.17  & 45.49   & 21.99  & 27.5                                                    \\
                                     & \textbf( +REINFORCE(BLEU))    & \textbf{46.66} & \textbf{31.09} & \textbf{22.80} & \textbf{17.31} & \textbf{46.27} & \textbf{22.06} &  \textbf{27.9} \\ \hline
\multirow{5}{*}{\textbf{MS-Marco}}   & \cite{learningtoask}                              & -               & -               & -               & 10.46           & -                & -               & -                                                                  \\ 
                                     & \cite{modelqgforqa}                              & -               & -               & -               & 11.46           & -                & -               & -                                                                  \\ 
                                     & \cite{para}^*            & -               & -               & -               & 16.02           & -                & -               & -                                                                  \\ 
                                     & EAD Model                & 51.39           & 33.48           & 22.92           & 16.57           & 50.34   & 24.89           &   25.6                                                                 \\ 
                                     & \textbf{RevNet Model}     & 52.18  & 33.93  & 23.93  & 17.01  & 50.30            & 25.13  & 25.7 \textbf{}                                                          \\
                                     & \textbf(+REINFORCE(BLEU))    & \textbf{52.64} & \textbf{34.55} &\textbf{ 24.07} & \textbf{17.60} & \textbf{50.97} & \textbf{25.51} & \textbf{26.2}\\ \hline
\end{tabular}
}
\caption{Comparison between our models and the existing works on $n$-gram metrics and answerability. *We refer to their Sentence Level Model}
\label{tab:results1}
\end{table*}


==> notused/results_and_discussions.tex <==
\section{Results and Discussions: EAD vs RevNet}
\label{sec:results}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
%\input{comparison_with_baselines}
%\input{revnet_on_other_datasets}
\input{all_datasets.tex}

In this Section, we present the results and analysis of our proposed model. Throughout this section, we refer to our models as follows
{\flushleft \bf Encode-Attend-Decode (EAD) model} is our proposed \bvscomment{our proposed?} single decoder architecture containing the encoder and the Preliminary Decoder described earlier.
{\flushleft \bf Revision Network (RevNet) model} which includes the encoder, the Preliminary Decoder and the Revision Decoder.\\

\subsection{RevNet's performance across datasets}
In table \ref{tab:results1}, we first compare the performance of our proposed models with the state-of-the-art models on the SQuAD dataset. Our RevNet model outperforms the baselines by $13.81$\% and $3.7$\% on BLEU-4 on SQuAD sentence and passage level question generation tasks. Also, our RevNet model is consistently better across all n-gram scores. It is to be noted that our EAD model also performs better than the state-of-the-art models in sentence level and performs almost equally in passage level.

We also evaluate our EAD and RevNet models on the HOTPOT-QA and DROP datasets. As discussed earlier, each of these dataset has a different style of questions and is more challenging than regular QA datasets. As shown in table~\ref{tab:results1} our RevNet model outperforms EAD for all styles of questions. For multihop (HOTPOT-QA) and reasoning (DROP) questions, RevNet model performs 7.6\% and 15.42\% better than the EAD models.Along with the N-gram scores, we evaluate the generated questions on Q-BLEU4 which gives a measure of both answerability and fluency. Our model also outperforms EAD model across all datasets in terms of Q-BLEU4 metric. 

\subsection{Human Evaluations to compare RevNet and EAD}
We also conducted human evaluations to analyze the quality of the questions produced by our \textbf{EAD} and \textbf{RevNet} models. We randomly sampled 500 generated questions from the SQuAD (sentence level) dataset and asked the annotators to compare the quality of the generated questions. 
    The annotator could choose if either of the question generated from EAD or RevNet model were better in terms of Fluency, Completeness, and Answerability. They were also allowed to skip the questions where they could not make a clear choice. Three annotators rated each question and the final label was calculated based on majority voting. We observed that the RevNet model outperforms the EAD model across all three metrics. Over 68.6\% of the questions generated by the RevNet model were more fluent than the EAD model. The RevNet model also produces 66.7\% more complete questions and 64.2\% answerable questions when compared to the EAD model. \bvscomment{while you are stating the result here, it is unclear why this should be right or significant. Have a couple of lines indicating on the 1/3rd cases where ours didn't make the cut.}

\input{analysis_of_revnet.tex}

\subsection{Visualization of Attention plots from $\mathbf{A_1}$, $\mathbf{A_2}$ and $\mathbf{A_3}$}
We plot the aggregated attention given to the passage and initial draft of the generation question across the various timesteps of the decoder in Figure \ref{attentionplots} for Example 2 in Table \ref{tab:generatedsamples1}. Although, both the questions are specific to the answer, $\mathbf{A_2}$ pays some attention to the context surrounding the answer, which leads to complete question. Also, note that in $\mathbf{A_3}$, while attending on to initial draft ``oncogenic'' word is not paid attention to and thus the final draft revises over the initial draft by correcting it to generate a better question.

\begin{figure}
\begin{subfigure}[b]{0.55\textwidth}
   \includegraphics[width=0.9\columnwidth]{d1-encoder.jpg}
   \caption{$\mathbf{A_1}$ attention plot}
   \label{fig:Ng1} 
\end{subfigure}
\begin{subfigure}[b]{0.55\textwidth}
   \includegraphics[width=0.9\columnwidth]{d2-encoder}
    \caption{$\mathbf{A_2}$ attention plot}
   \label{fig:Ng2}
\end{subfigure}
\begin{subfigure}[b]{0.55\textwidth}
   \includegraphics[width=0.9\columnwidth]{d1-d2}
   \caption{$\mathbf{A_3}$ attention plot}
   \label{fig:Ng2}
\end{subfigure}
\caption{Attention plots for a) $\mathbf{A_1}$, b) $\mathbf{A_2}$, c) $\mathbf{A_3}$ respectively \\
\textbf{Initial Generated Question}: ``What is the name of the oncogenic virus?'' \\
\textbf{Revised Generated Question}: ``What is the name of the organism that causes cervical\\ cancer?''}
\label{attentionplots}
\end{figure}



==> notused/results_and_discussions_reinforce.tex <==

%Motivation for this section: In the above sections we have discussed that adding a second revision improves the quality of the questions by making it elaborate . But the revision is not specific to any specific property. We try and model this by REINFORCE algorithm where we try to improve the quality of the question for two of the several aspect of the question: fluency and answerability, i.e. whethere the question arrives at the specific answer. For this we use our proposed REINFORCE Revision module and use BLEU and QBLEU as metrics to improve the question on each of the given metric. For both the metrics, we conduct human evaluations and show that these metrics are able to improve the quality of the question across these metrics both quantitatively and qualitatively. 
\section{Results and Discussions: REINFORCE Revision v/s RevNet}
\subsection {Comparison between REINFORCE Revision v/s RevNet }
In the above sections, although the quality of the revised questions is better than the initial draft, we were not explicitly training the model to be better in the second pass.  In this section, we explicitly train our model to generate better questions in the second pass, with respect to fluency and answerability.  We finetune the RevNet model using REINFORCE Revision module, with BLEU ad QBLEU as reward functions. Subsequently, we quantitatively and qualitatively analyze the impact of  REINFORCE Revision model over vanilla Revnet model. \\

We can infer from Table \ref{}, that the performance of the model improves with both BLEU ad QBLEU as reward functions across all the datasets, by  XX\%, XX\% and for SQuAD sentence level, SQuAD passage level, Hotpot and DRop datasets. We also conduct human evaluations to evaluate how each of the reward function BLEU and QBLEU impacts the fluency and answerability of the model. The procedure for collecting annotations was the same as one described in Section \ref{XX}. We sample 200 samples for each reward function for SQuAD sentence level dataset. We observe that for REINFORCE Revision (BLEU), annotators choose the fine-tuned questions XX\% in terms of fluency and XX\% in terms of answerability. The quality of the questions is slightly better with REINFORCE Revision (QBLEU) where the metric takes into account both fluency and answerability in its formulation. 
\subsection{Originality Analysis}

\begin{table}[h]
    \begin{tabular}{l}
        \hline 
         \textbf{Passage:} \textcolor{blue}{Cost engineers and estimators} apply\\ expertise to relate the work and materials \\
         involved to a proper valuation \\
         \hline 
         \textbf{Questions} \\
          \textit{Generated}: Who apply expertise to relate the work\\
           and materials involved to a proper valuation ? \\
          \textit{True}: Who applies expertise to relate the work \\
          and materials involved to a proper valuation ?\\
         \hline
    \end{tabular}
    \caption{An example of question with significant overlap with the passage}
    \label{tab:originality}
\end{table}

\begin{figure}
    \centering
    \includegraphics[scale=0.45]{qbleu_originality.png}
    \caption{Plot of Q-BLEU}
    \label{fig:qbleu_originality}
\end{figure}


We observe that current state-of-the-art models perform very well in terms of BLEU/QBLEU scores when the actual question has significant overlap with the passage. For example, consider a passage from the SQuAD dataset shown in table \ref{tab:originality} (answer in blue), where except for the question word \textit{who}, the model sequentially copies everything from the passage and achieves a Q-BLEU score of 92.4. However, the model performs poorly in situations where it has to draft questions in its own words. In order to quantify this, we first sort the true questions in the SQuAD test dataset based on its BLEU-2 overlap with the passage in ascending order. We then select the first $N$ data points to compute the QBLEU score between the generated and true questions. The results are shown in red in figure \ref{fig:qbleu_originality}, where the x-axis represents $N$ - the number points selected, and the y-axis represents the obtained QBLEU score. Towards the left, where there are true questions with low overlap with the passage, the performance\ is poor, and it gradually improves when questions with more considerable overlap are added.\\

The task of generating questions with high \textit{originality} (where the model phrases the question in its own words) is the challenging aspect of AQG since it requires complete understating of the semantics and syntactics of the language. In order to revise the questions towards \textit{originality}, we use RevNet with \textit{originality} specific rewards as discussed in the previous section. The results of the same experiment are shown in blue in figure \ref{fig:qbleu_originality}, we observe that Attribute-Guided RevNet performs better than RevNet especially in Questions which have low overlap with the passage.
 

==> notused/table_results_extra_dataset.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{Dataset}}      & \multirow{2}{*}{\textbf{Model}}                                 & \multicolumn{6}{c|}{\textbf{n-gram}}                                                                & \textbf{Answerability} \\ \cline{3-9} 
                                       &                                                                 & BLEU-1         & BLEU-2         & BLEU-3         & BLEU-4         & ROUGE-L        & METEOR         & Q-BLEU4                \\ \hline
\multirow{5}{*}{\textbf{HOTPOT}}       & EAD                                                             & 37.69          & 26.98          & 20.72          & 16.45          & 38.30          & 24.43          & 26.3                   \\
                                       & RevNet                                                          & 45.45          & 33.13          & 26.05          & 21.17          & 43.12          & 25.81          & 30.7                   \\
                                       & RevNet + BLEU                                                   & \textbf{}      & \textbf{}      & \textbf{}      & \textbf{}      & \textbf{}      &                &                        \\
                                       & RevNet + QBleu                                                  & \textbf{47.96} & \textbf{34.62} & \textbf{26.82} & \textbf{21.48} & \textbf{43.35} & \textbf{25.03} & \textbf{31.4}          \\
                                       & RevNet + Originality                                            & \textbf{48.73}          & \textbf{35.08}          & \textbf{27.13}          & \textbf{21.71 }         & \textbf{43.41 }         & 24.81          & 31.2                  \\ \hline
\multirow{5}{*}{\textbf{DROP Dataset}} & EAD                                                             & 39.21          & 29.10          & 22.65          & 18.42          & 45.07          & 19.56          & 31.8                   \\
                                       & RevNet                                                          & 42.81          & 32.63          & 25.78          & 21.23          & 47.49          & 22.25          & 33.6                   \\
                                       & RevNet+ BLEU                                                    & \textbf{42.82} & \textbf{32.83} & \textbf{26.12} & \textbf{21.60} & \textbf{48.16} & \textbf{22.43} & \textbf{34.3}          \\
                                       & RevNet + QBLEU                                                  & 42.66          & 32.73          & 26.06          & 21.59          & 47.83          & 22.29          & 34.1                   \\
                                       & RevNet + Originality & 42.98          & 32.91          & 26.11          & 21.56          & 47.90          & 22.43          & 34                     \\ \hline
\multirow{5}{*}{\textbf{MS-Marco}}     & EAD                                                             & 46.66          & 30.85          & 22.56          & 17.11          & 45.35          & 21.24          & 27.0                   \\
                                       & RevNet                                                          & 46.00 & 33.02 & 24.05 & 18.00 & 48.02          & 23.80 & 27.8          \\
                                       & RevNet +BLEU                                                    & \textbf{46.82}          & \textbf{33.98  }        & \textbf{25.05 }         & \textbf{18.90}          & \textbf{49.32} & \textbf{24.35}          & \textbf{28.8  }                 \\
                                       & RevNet + QBleu                                                  & 46.82          & 33.93          & 24.94          & 18.75          & 49.20          & 24.35          & 28.60                  \\
                                       & RevNet + Originality                                            &                &                &                &                &                &                &                        \\ \hline
\end{tabular}}
\label{tab:resultsextra}
\caption{Performance of RevNet model on HOTPOT, DROP and MS-Marco}
\end{table*}

==> notused/table_results_sentence_passage.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|lllllll|l|}
\hline
\multirow{2}{*}{\textbf{Dataset}}                                                          & \multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{6}{c|}{\textbf{n-gram}}                                                                                                                                                                         & \textbf{Answerability} \\ \cline{3-9} 
                                                                                           & \multicolumn{1}{l|}{}                                & \multicolumn{1}{l|}{BLEU-1}         & \multicolumn{1}{l|}{BLEU-2}         & \multicolumn{1}{l|}{BLEU-3}         & \multicolumn{1}{l|}{BLEU-4}         & \multicolumn{1}{l|}{ROUGE-L}        & METEOR         & Q-BLEU4                \\ \hline
\multirow{8}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}SQuAD\\ (Sentence Level)\end{tabular}}} & \multicolumn{1}{l|}{EAD}                             & \multicolumn{1}{l|}{44.74}          & \multicolumn{1}{l|}{29.79}          & \multicolumn{1}{l|}{22.00}          & \multicolumn{1}{l|}{16.84}          & \multicolumn{1}{l|}{44.78}          & 20.60          & 24.70                  \\
                                                                                          % & %\multicolumn{1}{l|}{EAD + BLEU}                      & \multicolumn{1}{l|}{46.21}          & \multicolumn{1}{l|}{31.22}          & \multicolumn{1}{l|}{23.25}          & \multicolumn{1}{l|}{17.94}          & \multicolumn{1}{l|}{46.04}          & 21.50          & 26.2                   \\
                                                                                          % & %\multicolumn{1}{l|}{EAD + QBLEU}                     & \multicolumn{1}{l|}{46.11}          & \multicolumn{1}{l|}{31.06}          & \multicolumn{1}{l|}{23.08}          & \multicolumn{1}{l|}{17.74}          & \multicolumn{1}{l|}{46.01}          & 21.37          & 26.1                   \\
                                                                                          % & %\multicolumn{1}{l|}{EAD + Originality}               & \multicolumn{1}{l|}{44.07}          & \multicolumn{1}{l|}{29.55}          & \multicolumn{1}{l|}{21.95}          & \multicolumn{1}{l|}{16.68}          & \multicolumn{1}{l|}{45.53}          & 20.61          & 25.5                   \\ \cline{2-9} 
                                                                 &                           \multicolumn{1}{l|}{RevNet}                          & \multicolumn{1}{l|}{47.27}          & \multicolumn{1}{l|}{31.88}          & \multicolumn{1}{l|}{23.65}          & \multicolumn{1}{l|}{18.16}          & \multicolumn{1}{l|}{47.14}          & 23.40          & 27.40                  \\
                                                                                           & \multicolumn{1}{l|}{RevNet + BLEU}                   & \multicolumn{1}{l|}{\textbf{48.17}} & \multicolumn{1}{l|}{\textbf{32.49}} & \multicolumn{1}{l|}{\textbf{24.12}} & \multicolumn{1}{l|}{\textbf{18.52}} & \multicolumn{1}{l|}{\textbf{47.56}} & 23.49          & 27.60                  \\
                                                                                           & \multicolumn{1}{l|}{RevNet + QBleu}                  & \multicolumn{1}{l|}{47.49}          & \multicolumn{1}{l|}{32.03}          & \multicolumn{1}{l|}{23.74}          & \multicolumn{1}{l|}{18.17}          & \multicolumn{1}{l|}{47.88}          & \textbf{23.87} & \textbf{28.60}         \\
                                                                                           & \multicolumn{1}{l|}{RevNet + Originality}            & \multicolumn{1}{l|}{46.84}          & \multicolumn{1}{l|}{31.55}          & \multicolumn{1}{l|}{23.37}          & \multicolumn{1}{l|}{17.90}          & \multicolumn{1}{l|}{47.57}          & 23.73          & 27.80                  \\ \hline
\multirow{8}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}SQuAD\\ (Passage Level)\end{tabular}}}  & \multicolumn{1}{l|}{EAD}                             & \multicolumn{1}{l|}{43.17}          & \multicolumn{1}{l|}{28.24}          & \multicolumn{1}{l|}{20.52}          & \multicolumn{1}{l|}{15.52}          & \multicolumn{1}{l|}{43.96}          & 19.74          & 24.2                  \\
                                                                                           %& %\multicolumn{1}{l|}{EAD + BLEU}                      & \multicolumn{1}{l|}{}               & \multicolumn{1}{l|}{}               & \multicolumn{1}{l|}{}               & \multicolumn{1}{l|}{}               & \multicolumn{1}{l|}{}               &                &                        \\
                                                                                           %& %\multicolumn{1}{l|}{EAD + QBLEU}                     & \multicolumn{1}{l|}{44.48}               & \multicolumn{1}{l|}{29.70}               & \multicolumn{1}{l|}{21.94}               & \multicolumn{1}{l|}{16.83}               & \multicolumn{1}{l|}{45.03}               &  20.63              &    25.4                   \\
                                                                                        %   & %\multicolumn{1}{l|}{EAD + Original}                  & \multicolumn{1}{l|}{43.17}          & \multicolumn{1}{l|}{28.24}          & \multicolumn{1}{l|}{20.52}          & \multicolumn{1}{l|}{15.52}          & \multicolumn{1}{l|}{43.96}          & 19.74         & 24.20                  \\ \cline{2-9} 
                                                                                           & \multicolumn{1}{l|}{RevNet}                          & \multicolumn{1}{l|}{46.41}          & \multicolumn{1}{l|}{30.66}          & \multicolumn{1}{l|}{22.42}          & \multicolumn{1}{l|}{16.99}          & \multicolumn{1}{l|}{45.03}          & 21.10          & 26.60                  \\
                                                                                         & \multicolumn{1}{l|}{RevNet + BLEU}                   & \multicolumn{1}{l|}{46.66}          & \multicolumn{1}{l|}{30.85}          & \multicolumn{1}{l|}{22.56}          & \multicolumn{1}{l|}{17.11}          & \multicolumn{1}{l|}{45.35}          & 21.24          & 27.0                   \\
                                                                                           & \multicolumn{1}{l|}{RevNet + QBLEu}                  & \multicolumn{1}{l|}{\textbf{46.83}} & \multicolumn{1}{l|}{\textbf{31.08}} & \multicolumn{1}{l|}{\textbf{22.76}} & \multicolumn{1}{l|}{\textbf{17.24}} & \multicolumn{1}{l|}{45.66}          & \textbf{21.32} & \textbf{27.20}         \\
                                                                                           & \multicolumn{1}{l|}{RevNet + Original}               & \multicolumn{1}{l|}{46.18}          & \multicolumn{1}{l|}{30.40}          & \multicolumn{1}{l|}{22.10}          & \multicolumn{1}{l|}{16.66}          & \multicolumn{1}{l|}{\textbf{45.68}} & 20.88          & 27.10                  \\ \hline

\end{tabular}}
\caption{Comparsion on SQuAD dataset }
\label{tab:results1}
\end{table*}
